Implant Global and Local Hierarchy Information to Sequence based Code Representation Models

Source code representation with deep learning techniques is an important research field. There have been many studies that learn sequential or structural information for code representation. But sequence-based models and non-sequence-models both have their limitations. Researchers attempt to incorporate structural information to sequence-based models, but they only mine part of token-level hierarchical structure information. In this paper, we analyze how the complete hierarchical structure influences the tokens in code sequences and abstract this influence as a property of code tokens called hierarchical embedding. The hierarchical embedding is further divided into statement-level global hierarchy and token-level local hierarchy. Furthermore, we propose the Hierarchy Transformer (HiT), a simple but effective sequence model to incorporate the complete hierarchical embeddings of source code into a Transformer model. We demonstrate the effectiveness of hierarchical embedding on learning code structure with an experiment on variable scope detection task. Further evaluation shows that HiT outperforms SOTA baseline models and show stable training efficiency on three source code-related tasks involving classification and generation tasks across 8 different datasets.

==> chapter/abstract.tex <==
\begin{abstract}
Source code representation with deep learning techniques is an important research field.
Sequence models, such as Transformer, have produced excellent and efficient performance across different source code-related tasks, but are sub-optimal for capturing structural information.
\TODO{modify}
% , based on the ``naturalness'' of programming languages.
% However, sequence models are inherently skilled at processing linear text and sub-optimal for capturing structural information. 
Existing non-sequence-based methods such as tree-based or graph-based models focus on how to encode structural information, but ignore the alignment and fusion of structural information and sequence information, thus sacrificing the advantages of sequence models. Our key insight is to incorporate and align structural information into sequence models with minimal additional cost.
% \TODO{add non sequence models}
% \TODO{align information}
% it is difficult for sequence models to capture the hierarchical structure of source code,
% combine the hierarchical structure of source code with naturalness

In this paper, we demonstrate that the hierarchical position can be used as a bridge to align semantic structure and sequence information of source code. 
% Modeling the hierarchical structure in source code is essential for understanding the semantics of programs through deep analysis.
% Hierarchical structure complements sequence   
% order information in source code, and influence the token-level semantics, statement-level semantics, and even the whole program functionality.
We propose the \textbf{Hi}erarchy \textbf{T}ransformer (HiT), a simple but effective sequence model to incorporate hierarchical position of source code 
% into a concise Transformer format.
into a Transformer model.
% HiT consists of two key parts: a Hierarchy Encoder and a Sequence Encoder.
% The Hierarchy Encoder extracts the hierarchical position from paths in the concrete syntax tree.
% Then the Sequence Encoder encodes the hierarchy representation and original token sequence jointly. 
HiT takes advantage of sequence models and learns the hierarchical structure well yet.
% Hierarchy extraction 
% modify transformer
\TODO{modify}
Experiments show that modeling the hierarchical position significantly enhances the capacity of sequence models with a cost of only 1\%-5\% additional parameters.
% Compared with Transformer, HiT improves the accuracy by over 25\% on the C++1400 classification dataset and MAP@R by over 13\% on the POJ clone detection dataset.
% we claim the importance of modeling hierarchy for code representation and prove it through an in-depth evaluation.
Furthermore, HiT shows stable excellent and stable training efficiency, and outperforms SOTA baseline models, including tree-based models (TBCNN, TreeCaps) and graph-based models (GGNN, GREAT)
on three source code-related tasks involving classification and generation tasks across 8 different datasets.
% The evaluation demonstrates the superiority of modeling "naturalness" with "hierarchy"
\end{abstract}


==> chapter/abstract_v1.tex <==
\begin{abstract}
    Source code representation with deep learning techniques is an important research field in the past few decades. 
    Researchers have demonstrated the ``naturalness'' of programming languages that programs written in real world scenarios are repetitive and have predictable properties. 
    Sequence models such as LSTM and Transformer 
    % have been popular models applied for source code related tasks due to the ``naturalness'' of programming languages.
    % Programming languages are known to have ``naturalness'': the programs written in real world scenarios are repetitive and have predictable properties. Thus source code can be modeled by neural networks designed for understanding sequence input such as LSTM and Transformer.
    % Sequence models 
    are producing great performance across different source code related tasks.
    However, when capturing ``naturalness'' of source code, these models overlook an important feature: source code is hierarchical instead of a linear text.
    The semantics of statements and code tokens are influenced by their hierarchical position in the program.
    In this paper, we claim the importance of modeling hierarchy for code understanding and prove it through detailed experiments.
    % We divide the location of source code tokens to two location concepts, absolute location and relative location, where absolute location refers to the hierarchical position of the statement and relative location refers to the location of a token in the statement.
    We design a simple but effective model, the \textbf{Hi}erarchy \textbf{T}ransformer (HiT), to incorporate hierarchicy information into sequence understanding models. Further experiments show that the simple augmentation on Transformer results in a SOTA code representation model. Our proposed HiT outperforms strong baseline models on three code understanding tasks involving classification and generation tasks across 8 different datasets.
\end{abstract}


==> chapter/background.tex <==
To better present the methodology of our model, we first provide some background and preliminaries in this section, including a brief introduction to the popular sequence model Transformer and syntax parsing trees of source code.
The employed symbols are summarized in Table \ref{tab:notation}.
% In this section, we give a brief introduction to the classical sequence model, including LSTM, Transformer, \etc. To better illustrate our approach, we also give a basic introduction to the Concrete Syntax Tree (CST) of the source code.


\input{table/symbols}

% \subsection{Deep Models for Sequence Modeling}

% \paragraph{RNN and its variants}
% Recurrent Neural Network (RNN) \cite{ZarembaSV14RNN} and its variants have been the most popular model for encoding sequential data. Given the input token sequence $s = (t_1, t_2, \cdots, t_l)$, the input of an RNN model is usually the word embeddings $(e_1, e_2, \cdots, e_n)$. RNN encodes the input tokens one by one with the formula:
% \begin{equation}
%     \begin{aligned}
%     h_t &= f(W_1e_t + W_2h_{t-1} + b) \\
% \end{aligned}
% \end{equation}
% where $f, g$ is nonlinear activation functions such as $tanh$ and $W, b$ are learnable parameters..
% RNN is a dedicated model for sequence data and learns the sequential relation of the input tokens well. However, RNN faces a big issue when modeling long input sequences: the gradient vanishing and gradient exploding \cite{HochreiterS97LSTM}. Researchers propose GRU \cite{ChoMGBBSB14GRU} and LSTM \cite{HochreiterS97LSTM} to solve this issue. GRU and LSTM are the most used variants of RNN. They ease the gradient vanishing and exploding problem by employing gate mechanisms. However, the long-time dependency problem in sequence modeling is still not fully addressed \cite{khandelwal2018sharp}. Later, \citea{vaswani2017attention} proposes Transformer, which utilizes the self-attention mechanism and adds direct connections between token pairs at arbitrary positions and solves the problem well.

\subsection{Transformer}

Transformer \cite{vaswani2017attention} is a model architecture relying on the attention mechanism. Given input tokens $\{x_i\}_{i=1}^{\left | x \right | }$, we pack their word embeddings to a matrix $X^0 = \left [ x_1,\dots ,x_{\left | x \right | } \right ] $. The stacked $L$-layer Transformer computes the final output based on embeddings via $X^{l} = \operatorname{Transformer}_l(X^{l-1}), l \in \left [1,L \right ]$.
The core component of a Transformer block is multi-head self-attention. The $h$-th self-attention head is described as:
% $$Q_{h}=X W_{h}^{Q}, K=X W_{h}^{K}, V=X W_{h}^{V} $$
% $$A_{h}=\operatorname{softmax}\left(\frac{Q_{h}K_{h}^{\top}}{\sqrt{d_{k}}}\right)
% $$
% $$H_{h}=\text { AttentionHead }(X)=A_{h} V_{h}$$
\begin{equation*}
\begin{aligned}
Q_{h}=X W_{h}^{Q}, K=X W_{h}^{K}, V=X W_{h}^{V} \\
% \end{equation}
% \begin{equation}
A_{h}=\operatorname{softmax}\left(\frac{Q_{h} K_{h}^{\top}}{\sqrt{d_{k}}}\right) \\
% \end{equation}
% \begin{equation}
H_{h}=\text { AttentionHead }(X)=A_{h} V_{h}
\end{aligned}
\end{equation*}

where $Q,K \in {\mathbb{R}}^{n \times d_k}, V \in {\mathbb{R}}^{n \times d_v} $, and the score $A_{i,j}$
indicates how much attention token $x_i$ puts on $x_j$.
There are usually multiple attention heads in a Transformer block. The attention heads follow the same computation despite using different parameters.
Let $\left | h \right |$ denotes the number of attention heads in each layer, the multi-head attention output is given by $\operatorname{MultiHead}(X) = \left [ H_1 || \cdots || H_{\left | h \right |} \right ]W^{o}$,
where $W^o \in {\mathbb{R}}^{\left | h \right |d_v \times d_x}$,
 $||$ means concatenation.

\subsection{Parsing Tree}

A parsing tree of source code is an ordered tree that represents the syntactic structure according to the context-free grammar of the programming language.
Parsing trees contain rich structural information of source code. They can be acquired with existing parsers easily. 
Concrete syntax tree (CST) and abstract syntax tree (AST) are parsing trees. The concrete syntax tree reflects the exact syntax of the source code, where each leaf node corresponds to a source code token. In theory, a CST can be converted to an AST equivalently. However, ASTs do not represent every detail appearing in the real syntax. For instance, the braces, semicolons, and parentheses are discarded in ASTs, making it hard to align the structural information with these code tokens. To extract the hierarchical position of each source code token, we use CSTs in this work.



==> chapter/intro_deprecated.tex <==

% code representation
% 结果信息在代码中很重要
% 现有的编码AST的工作:
%  序列化AST： SBT, X-SBT(SPT-Code: Sequence-to-Sequence Pre-Training for Learning Source Code Representations)
%  code2vec, code2seq
%  GNN

% 现有方法存在的问题:
% 未能将词法的序列信息和结构的层次信息结合起来考虑
% code tokens词法信息，paths结构信息
% GNN感受野小, 也不能建模长距离的层次信息和序列信息
% (leaf-to-leaf path和root-to-leaf path的效率问题?)


% 故事1
% 深度学习在程序表示上的应用，程序表示的目标是将程序转化为向量表示，程序表示可以用于很多任务中，诸如xxx，程序表示模型潜力巨大，被广泛应用

% 考虑到序列模型成熟的强大能力，一种简单的方法是将程序语言编码为序列进行建模，利用seq2seq的模型进行建模，类似的工作被广泛地采用，并在诸多领域的子任务上达到了很好的效果。然而程序语言具有丰富的结构信息，给定一段代码[token1, token2, ...,]，相同的n可能运行在不同的环境中，定义在不同的作用域中，从而具有截然不同的语义信息。
% 画一个图，相同的变量，不同的作用域，以及对应的AST中的path

% 为了解决这一问题，在本文中，我们提出在序列编码中需要包含作用域信息。为了获取到token的作用域信息，我们从AST中挖掘root-to-leaf的path信息作为scope信息并进行表示。（根据图来详细解释一下，诸如path中的pattern等）。我们将scope信息和token信息综合考虑，从而形成新的代码的序列表示。

% 受益于transformer模型的高效建模序列的能力，我们首先使用获得scope的表示，再将其combine在序列token上。通过极小的代价（模型参数和效率？），我们显著提升了序列表示模型的能力。
% 同时，我们也将我们的模型和众多结构相关的表示模型诸如xxx，以及其他sota模型相比较。我们在多个任务数据集上进行测试，结果显著提高，证明了我们方法的有效性。



% 故事2

% Incorporating Structural Positional Embedding for Code Understanding

% 深度学习在程序表示上的应用，程序表示的目标是将程序转化为向量表示，程序表示可以用于很多任务中，诸如xxx。

% Transformer作为NLP中的SOTA模型，应用广泛。程序语言和自然语言有一定的相似性，很多工作将code看作token序列，采用与处理自然语言同样的方法利用Transformer来编码code。但程序语言与自然语言一个重要的不同点在于强结构性，相比于常被看作顺序序列的自然语言，程序语言通常有更多层次的嵌套结构，所以将一般的序列模型运用到程序表示中去时，这样的结构性就会丢失。

% 比如
% ```
%     for i in range(10):
%         x += 1
%     print(x)
%         
% ```
% 第二个x和第一个x的序列距离虽然很近，但他们的结构距离实际上相差很多（一个在循环体内，一个在外）
% 再比如，两个函数定义func1, func2，很多情况下交换他们定义的位置并不会影响代码的语义，但是却很大程度影响了他们的位置编码。
% 所以我们设计了一种带结构信息的位置编码，加入序列x模型中，让它更好地学到代码表示。

% 句子与句子之间逻辑连起来

% Code representation介绍
Code representation is a hot research topic in both the software engineering (SE) and machine learning (ML) fields. Machine learning for code representation learning aims to convert programs of different formats (token sequences, abstract syntax trees, or dependency graphs, \etc) into vectorized semantic embeddings. These representation vectors are essential in source code processing and can be applied in many downstream tasks, such as code classification \cite{?}, clone detection \cite{?}, code summarization \cite{?}, method name prediction \cite{?}, \etc. A good code representation model can facilitate the development of various machine learning-based software tools.
Thus, many researchers have explored ways to design better code representation models.

% code representation model 大部分采用sequence model的方法
Most existing studies adopt sequence modeling architectures to represent source code, and achieve SOTA results on many code understanding tasks, e.g., code classification, code summarization, and program translation. 
Programming languages can be understood and manipulated with the same approaches as natural languages, based on the concept of ``naturalness''.
% Researchers can take different views of source code, e.g., code tokens, abstract syntax trees (AST), concrete syntax trees (CST), and data flow graphs (DFG).
\cite{naturalness} first propose the concept of ``naturalness'' for source code that programs written in real world scenarios are usually simple, repetitive, and have predictable statistical properties. They implement a completion engine for Java with a simple n-gram model and show the power of ``naturalness'', which implies the potential of modeling source code as token sequences.
Furthermore, in many source code related tasks, such as code completion, the input inherently takes the form of a sequence.
% Thus, sequence modeling architectures such as LSTM and Transformer have been very popular in the SE community.
These sequence models are producing appealing results on many code understanding tasks, e.g., code classification, code summarization, and program translation.
Furthermore, modeling source code as a token sequence requires for minimum cost of preprocessing compared with data-flow-based or graph-based methods.
% In many source code understanding tasks, the code snippet input takes the form of a sequence.


% According to the \cite{naturalness}, source code have the property named ``naturalness'': although programming languages are complex in theory, the programs written in real world scenarios are rather simple and repetitive. Thus they have predictable statistical properties which can be captured by language models.

% Then in lots of following code understanding work, researchers take code snippets input as the form of token sequence. They model source code tokens with promising sequence models such as RNN, LSTM, and Transformer, which have achieved state-of-the-art results across many natural language processing tasks.
% nice performance, codebert, xx
% some argue that syntactic, xxx
% ast, gnn
% preprocess, time efficiency, naturalness
% https://arxiv.org/pdf/2002.05442.pdf

% \TODO{add formal definition}
% Consequently, it is straightforward to model source code as a sequence of tokens just like considering natural language as a sequence of words.
% Source code is formed by a sequence of statements, similar to sentences in natural language. The statement is composed of tokens in source code, similar to words in natural language.
% Statement <-> Sentence, Token <-> Word. ...
% relationship is not as sim/ple as the relationship between \textit{\textbf{sentences}} and \textit{\textbf{words}} in natural language.

% Considering that researchers in the NLP community have witnessed the power of sequence models, 
% recently many studies have widely adopted the sequential modeling approach for code representation and achieved state-of-the-art results across many software engineering tasks, including code summarization \cite{?}, method name recommendation \cite{?}, code generation \cite{?}, program translation \cite{?}, \etc.
% However, it cannot be ignored that the location of different statements and different tokens cannot be simply organized as a sequential structure.
% \TODO{
% However, there are two important differences between source code and natural languages.
% }

% \begin{tcolorbox}[colback=white,size=title,breakable]
%     \quad tseto
% \end{tcolorbox}

\begin{figure}[t]
 \subfigure[Hierarchical location affects the operational semantics of a statement] {
  \label{fig:statement}     
  \includegraphics[width=\columnwidth]{fig/statement.pdf}  
  }

 \subfigure[Hierarchical position within a statement affects the semantics of a token.] {
  \label{fig:locality}     
  \includegraphics[width=\columnwidth]{fig/intro_loc.pdf}  
  }
\caption{An illustrative example of the hierarchy information in source code. The hierarchy of a token refers to the hierarchical location of its statement (\textit{global hierarchy}) and the local component of the token in the statement (\textit{local hierarchy}). The token \definenode{source\_i} and \definenode{value} are both \definenode{identifier} in \definenode{if\_comparison} marked in green in (b), and they are more closely related.}
\label{fig:intro_locality}
\end{figure}

Sequence models are performing well on source code understanding tasks based on the concept of ``naturalness''.
However, programs are still more complicated than linear texts which we read and write from left to right. It cannot be ignored that most programming languages have hierarchical structures. The semantics of programs are influenced by the hierarchical structure to a large extent. 
We illustrate this influence from two aspects of hierarchical structure:
\ding{182} Hierarchical position of statements (named as \textit{global hierarchy}).  The hierarchical position will affect the operational semantics of a statement. For example, in Figure \ref{fig:intro_locality}, the statement \definenode{count += 1} is written in the \definenode{for-block} and possibly to be executed more than once, while the statement \definenode{count = 0} will be executed only once in each function call to \definenode{countOccurrences}.
\ding{183} Hierarchical position of tokens within a statement (named as \textit{local hierarchy}). Tokens are in different components in a statement, which will affect the semantics of each token. \Eg, as shown in Figure \ref{fig:locality}, \definenode{if-statement} contains \definenode{if-comparison} component and \definenode{if-block} component.
There are three identifiers, \textit{source\_i},  \textit{value}, and \textit{count}, in the \definenode{if-statement}. All of them are references to a variable in the function. However, the first two identifiers within \definenode{if-comparison} component (marked in green color in the figure) have more similar semantics than \textit{count} because they appear in the same comparison expression.
% the distances between neighboring identifiers in the sequence are both 2 and we cannot directly identify the different roles of these three identifiers.

The hierarchical structure of source code is difficult for a simple sequence model to capture. When we flatten the input source code to a token sequence, the nested hierarchical structure is implicitly expressed by indentations for languages such as Python or brackets for languages such as Java and C/C++. We claim that it is important to model the hierarchy of programs in code understanding tasks and it is sub-optimal to learn this information from token sequences.
% Furthermore, the structure with in a statement is totally lost.


% In Figure \ref{fig:intro_locality}, \definenode{count}$^\text{\ding{172}}$ is assigned with a value

% Because of the syntactic structure of programming languages, the implicit local information changes for statements and tokens beyond sequence order. 
% \ding{182} Statements can be divided into several categories by its syntax or grammar, including \definenode{if-statement}, \definenode{for-statement}, \etc. Statements of different types are nested within each other to form code blocks with different functional semantics. Therefore, it is essential to determine the type and nesting relationship of a statement.
% \ding{182} The location of different statements are restricted by grammar rules and are divided into \definenode{if-statement}, \definenode{for-statement}, \etc. 
% \ding{183} The components of each token in the statement are also strictly defined. The connection between tokens in the same statement is generally closer, and this relationship is related to the components of each token.
% \Eg, \definenode{if-statement} may contain \definenode{if-comparison} component and \definenode{if-block} component respectively, and those identifier tokens in \definenode{if-comparison} are generally more related and comparable.
% Figure \ref{fig:statement} shows an example about this implicit local information beyond the sequence order for a piece of code. We can see that the location relationship at the statement level is expanded hierarchically and each token in the statement belongs to a specific component such as \definenode{if-comparison}.

% To this end, we propose the property of \textbf{locality} in code sequences. The locality refers to the location of each statement and its nesting relationship in the code structure (named as \textit{absolute locality}), and the local component of each token in a statement (named as \textit{relative locality}). Thus, we can define the locality property of each token, including the absolute locality of the statement to which it belongs and the relative locality of the token itself.
% To mine the locality information of source code, we focus on the hierarchy in the concrete syntax tree. 
% Each terminal node in the concrete syntax tree refers to a token in the code sequence, and each path from the root node to the terminal node refers to the locality information of a token in the code structure. 
% We divide the path into two parts according to the statement node closest to the leaf node, representing \textit{absolute locality} and \textit{relative locality} respectively.
% For example, we shows the root-to-leaf path of the source code token in Figure \ref{fig:locality}. The same token \definenode{count} in Figure \ref{fig:statement} has different locality, occurs in different statement, acts as different local components and thus has very different semantic information.


To validate our intuition of modeling the hierarchy of source code, we propose \textbf{Hi}erarchy \textbf{T}ransformer (HiT), a simple but effective method to incorporate hierarchy information into the code sequence representation model.
To extract the hierarchy of source code, we first parse the input code into a concrete syntax tree. The nested hierarchy can be represented by a path in the syntax tree. We use these syntax tree paths as additional hierarchy information to the sequence input. The HiT model consists of two key components: a Transformer-based hierarchy encoder that learns the representation of the hierarchical structure, and a Transformer-based sequence encoder that fuses the hierarchy information and token sequence information.
Note that our model can be regarded as a general way to augment a sequence-based code understanding model. It is trivial and direct to extend our model to other sequence models such as RNN and LSTM. We choose Transformer here because they have achieved state-of-the-art results in various NLP and source code related tasks.

% Since Transformers have achieved state-of-the-art results in various NLP tasks, we make a small modification to the Transformer model and nest a small Transformer in the vanilla Transformer model. The locality representation for each token is added in a concise Transformer format.
We conduct an empirical study to investigate the impact of the global and local hierarchy. The experiment proves the effectiveness of the two different types of hierarchy information. It shows that with the cost of a small number of additional parameters, our approach significantly enhance the performance of sequence-based code representation models.
We further evaluate our approach on three tasks: code classification, clone detection and method name prediction, with 8 different datasets from different domains. These tasks include classification tasks and generation tasks in the field of source code processing.
% , and both of them requires understanding the semantics of the input code snippets.
The experimental results show that our approach outperforms existing structure-based code representation models and other state-of-the-art models, indicating the benefits of our approach for combining "naturalness" and "hierarchy" for source code understanding.

The main contributions of this paper are summarized as follow.
\begin{itemize}[leftmargin=*]
    \item We claim the influence of hierarchy on the semantics of source code, which include the hierarchy of the statements (named as global hierarchy) and the hierarchy with in a statement (named as local hierarchy) in the code structure. % The hierarchy information is complementary to the token sequence information of source code.
    \item We propose a simple but effective approach to incorporate the hierarchy information to the Transformer model. With the cost of a small number of additional parameters, our approach significantly improve the performance of code sequence representation models. We also conduct an empirical study exploring the effectiveness of the two different kinds of hierarchy information.
    \item We evaluate our approach on three different tasks with 8 different datasets, involving classification tasks and generation tasks on source code. Our approach generally outperforms models on most of the tasks, showing excellent performance. Our experimental results prove that combining "naturalness" and "hierarchy" is effective for learning representations for programs.
\end{itemize}

% Source code is formed by a sequence of one or more \textit{statements}, which performs as the syntactic unit. 
% The type of the \textit{\textbf{statement}} and its position in the program are different, and the components of the \textit{\textbf{token}} within the statement are also different. Due to the structure of programs, this 
% To this end, we propose the property of \textit{locality} of okens in code sequences.
% The locality of source code refers to the 
% The locality of source code refers to the fact that the semantic of a token or statement is related to the location and context. In other words, the locality determines the location and context information of a token in the code structure.
% Given a sequence of source code $s = [token_1, token_2, \dots, token_n]$, the same $token$ may have different locality, run in different environments/blocks, defined in different scopes, acted as different compositions and thus have very different semantic information. For the same reason, different tokens may also have more similar localities. For instance, Figure \ref{?} shows a piece of source code, illustrating the different changing relationships between token and locality.
% \TODO{add some explaination}
% def distance(x0, y0, x1, y1):
    % x0 = pow(abs(x0 - x1), 2)
    % y0 = pow(abs(y0 - y1), 2)
    % return sqrt(x0 + y0)



% \me{To tackle the issue of the "ambiguous" token in code sequence representation, } 
% To tackle the issue of tokens with unclear locality, we propose to explore the approach to incorporate locality into the sequence representation model of source code. We add additional locality information to each token so that the sequence representation of the code turns into $s^{new} = [(locality_1,token_1), (locality_2,token_2), \dots, (locality_n,token_n)]$.

% Thanks to the power of the sequence model,  it is an effective and direct approach to 
% Thanks to the powerfulness of deep learning, representations of code can be obtained via a variety of deep neural networks. 
% In order to obtain better code representations, researchers have incorporated structural information into the modeling process -- from the trivial token sequences \cite{DBLP:journals/neco/HochreiterS97,DBLP:conf/emnlp/ChoMGBBSB14}, to the abstract syntax trees (AST) \cite{DBLP:conf/aaai/MouLZWJ16,DBLP:conf/icse/ZhangWZ0WL19,DBLP:journals/pacmpl/AlonZLY19,alon2018code2seq} and finally to the graphs \cite{allamanis2018learning,fernandes2018structured,brockschmidt2018generative,yin2018learning,allamanis2020typilus}.


% 结合树结构信息的工作
% 在AST上的工作，以及在transformer上的处理
% Considering that the structural information of programming language is stronger than that of natural language, recently researchers are now focusing more on how to encode the structural information of programs in better ways. 
% Some studies use the flattened abstract syntax tree (AST) node sequence as input to model the structure in source code. SBT \cite{1} traverse an AST and represents the tree nodes into a token sequence, thus uses a sequential model such as LSTM to model the structure information. X-SBT \cite{1} simplifies the SBT approach, optimizing and shortening the length of the sequence representation by using an XML-like form. 
% \me{Some works leverage the program AST to model the structure in source code and linearize the graph by traversing it. Code2seq represents source code as a set of pairwise paths over AST where each path is compressed to a vector using LSTMs [Hochreiter and Schmidhuber, 1997]. Code2seq obtains state-of-the-art for code representation using only AST information, demonstrating the effectiveness of path encoding. }
% \me{On the other hand, several works also leverage structured graph neural networks for modelling source code directly. [Allamanis et al., 2017] used Gated Graph Neural Network (GGNN) to embed the semantically meaningful relationships in the code. [Zhou et al., 2019] proposed a novel graph neural network with composite programming representation for vulnerability identiﬁcation. However, GNNs typically rely on synchronous message passing, requiring message passing iterations to aggregate information [Allamanis et al., 2017, Fernandes et al., 2018]. Besides, primarily for computational reasons, GNNs for programs usually compute few message-passing iterations. For these reasons, the representation of GNNs tends to be local and struggle to leverage long-range interactions.}

% However, these studies meets some problems: Existing models lack the ability to combine lexical sequential information with structural hierarchical information. Both the flatten AST node sequence and the set of pairwise paths over AST impair or lose the sequence information of the context of the source code. In the flatten AST node sequence, the sequential information of leaf nodes (indicating the lexical sequential information) is interspersed with other non-terminal nodes. In Code2seq, the context of source code are ignored. As for GNNs, the number of nodes in the receptive field of each node grows exponentially, which leads to GNNs not being able to understand the complete sequence information and structure information well. 

% % 使用transformer编码树结构的既有工作，以及存在的问题
% There are also some studies devoted to representing structural information using Transformer models. 
% \me{Transformer [Vaswani et al., 2017] allows global information ﬂow at each step but lacks the ability to model the structural complexity of source code. Recently, some works have explored introducing structural inductive bias in Transformers to access the global structural representation of source codes. [Hellendoorn et al., 2019] proposed Graph Relation Embedding Attention Transformer (GREAT), which extends [Shaw et al., 2018] and biases Transformer with relational information from graph edge types. After that, [Zügner et al., 2021] proposed Code Transformer based on the backbone of XLNet in [Yang et al., 2019], which computes pairwise distances on AST and integrate multiple relations into the attention module.}

% To overcome these drawback shown in previous studies, we adopt the ideas of encoding path to represent source code and propose an effective approach, \method{}, which intergrate the \textbf{tree} structural information \textbf{in} sequential \textbf{Transformer} encoder-decoder architecture. In order to make the transformer model can handle both hierarchical and sequence information, we nest a new small Transformer in the vanilla Transformer model to process the hierarchical information.
% We employ root-to-leaf paths in AST to represent the hierarchical structural information.
% and use a small Transformer model to process these information.
% considering that leaf-to-leaf paths calculation is too complicated. (Given a full binary tree of depth $d$, the number of all leaf-to-leaf paths is $2^{2n-2}$) 
% These structural information is combined with the corresponding leaf nodes to form a sequence to process the lexical sequential information. 
% \TODO{}



==> chapter/intro_new.tex <==

% code representation
% 结果信息在代码中很重要
% 现有的编码AST的工作:
%  序列化AST： SBT, X-SBT(SPT-Code: Sequence-to-Sequence Pre-Training for Learning Source Code Representations)
%  code2vec, code2seq
%  GNN

% 现有方法存在的问题:
% 未能将词法的序列信息和结构的层次信息结合起来考虑
% code tokens词法信息，paths结构信息
% GNN感受野小, 也不能建模长距离的层次信息和序列信息
% (leaf-to-leaf path和root-to-leaf path的效率问题?)


% 故事1
% 深度学习在程序表示上的应用，程序表示的目标是将程序转化为向量表示，程序表示可以用于很多任务中，诸如xxx，程序表示模型潜力巨大，被广泛应用

% 考虑到序列模型成熟的强大能力，一种简单的方法是将程序语言编码为序列进行建模，利用seq2seq的模型进行建模，类似的工作被广泛地采用，并在诸多领域的子任务上达到了很好的效果。然而程序语言具有丰富的结构信息，给定一段代码[token1, token2, ...,]，相同的n可能运行在不同的环境中，定义在不同的作用域中，从而具有截然不同的语义信息。
% 画一个图，相同的变量，不同的作用域，以及对应的AST中的path

% 为了解决这一问题，在本文中，我们提出在序列编码中需要包含作用域信息。为了获取到token的作用域信息，我们从AST中挖掘root-to-leaf的path信息作为scope信息并进行表示。（根据图来详细解释一下，诸如path中的pattern等）。我们将scope信息和token信息综合考虑，从而形成新的代码的序列表示。

% 受益于transformer模型的高效建模序列的能力，我们首先使用获得scope的表示，再将其combine在序列token上。通过极小的代价（模型参数和效率？），我们显著提升了序列表示模型的能力。
% 同时，我们也将我们的模型和众多结构相关的表示模型诸如xxx，以及其他sota模型相比较。我们在多个任务数据集上进行测试，结果显著提高，证明了我们方法的有效性。



% 故事2

% Incorporating Structural Positional Embedding for Code Understanding

% 深度学习在程序表示上的应用，程序表示的目标是将程序转化为向量表示，程序表示可以用于很多任务中，诸如xxx。

% Transformer作为NLP中的SOTA模型，应用广泛。程序语言和自然语言有一定的相似性，很多工作将code看作token序列，采用与处理自然语言同样的方法利用Transformer来编码code。但程序语言与自然语言一个重要的不同点在于强结构性，相比于常被看作顺序序列的自然语言，程序语言通常有更多层次的嵌套结构，所以将一般的序列模型运用到程序表示中去时，这样的结构性就会丢失。

% 比如
% ```
%     for i in range(10):
%         x += 1
%     print(x)
%         
% ```
% 第二个x和第一个x的序列距离虽然很近，但他们的结构距离实际上相差很多（一个在循环体内，一个在外）
% 再比如，两个函数定义func1, func2，很多情况下交换他们定义的位置并不会影响代码的语义，但是却很大程度影响了他们的位置编码。
% 所以我们设计了一种带结构信息的位置编码，加入序列x模型中，让它更好地学到代码表示。

% 句子与句子之间逻辑连起来

% Code representation介绍
Code representation is a hot research topic in software engineering (SE) and machine learning (ML) fields. Machine learning for code representation learning aims to convert programs of different formats (token sequences, abstract syntax trees, dependency graphs, \etc) into vectorized semantic embeddings. These representation vectors are essential in source code processing and can be applied in many downstream tasks, such as code classification \cite{tbcnn}, type inference \cite{allamanis2020typilus}, method name prediction \cite{code2vec,alon2018code2seq}, code summarization \cite{IyerKCZ16codenn,hu2018deep}, \etc. 
% A good code representation model can facilitate the development of various machine learning-based software tools.
% Therefore, many researchers have explored ways to design better code representation models.

\begin{figure}[t]
 \subfigure[Hierarchical location affects the operational semantics of a statement] {
  \label{fig:statement}     
  \includegraphics[width=\columnwidth]{fig/statement.pdf}  
  }

 \subfigure[Hierarchical position within a statement affects the semantics of a token.] {
  \label{fig:locality}     
  \includegraphics[width=\columnwidth]{fig/intro_loc.pdf}  
  }
\caption{An illustrative example of the hierarchical position in source code. The hierarchy of a token refers to the hierarchical location of its statement (\textit{global hierarchy}) and the local component of the token in the statement (\textit{local hierarchy}). The token \definenode{source\_i} and \definenode{value} are both \definenode{identifier} in \definenode{if\_comparison} marked in green in (b), and they are more closely related.}
\label{fig:intro_locality}
\end{figure}
% code representation model 大部分采用sequence model的方法
% Sequence modeling architectures are widely adopted in code representation learning
% % , based on the concept of ``naturalness`` 
% \cite{naturalness2012, AllamanisBDS18naturalness, cbert}, 
% which argues that programming languages are usually simple, repetitive, and can be understood through the same approaches used in natural language processing. 
% Many existing studies in code representation learning adopt sequence modeling architectures with the same approaches as natural languages, based on the concept of ``naturalness'',
% which indicates that programs written in real-world scenarios are usually simple, repetitive, and have predictable statistical properties.
% \cite{naturalness} first propose the concept of ``naturalness'' for source code that programs written in real-world scenarios are usually simple, repetitive, and have predictable statistical properties. They implement a completion engine for Java with a simple n-gram model and show the power of ``naturalness'', which implies the potential of modeling source code as token sequences.
% are popular and efficient code representation approaches that 

Sequence modeling architectures are widely adopted in code representation learning
% , based on the concept of ``naturalness`` 
\cite{naturalness2012, AllamanisBDS18naturalness, cbert}, 
and  can produce appealing and efficient results on source code-related tasks.
% Sequence models are popular,但存在一个重要的问题，即很难将层次结构编码进去
However, traditional sequence models are inherently skilled at processing linear text, but programs are more complicated than linear sequences and have complex semantic structures with different properties to source code.
There have been some attempts to encode structural information with sequence models, such as feeding the set of pairwise paths over AST \cite{code2vec, alon2018code2seq} or the traversal sequences of ASTs \cite{hu2018deep, SPTCode}.
Others utilize tree-based models \cite{tbcnn,icseZhangWZ0WL19astnn,aaaiBuiYJ21treecaps} and graph-based models \cite{allamanis2018learning} to capture structural information.
These methods can capture the semantic structure of programs, but discard the code sequence or intersperse code tokens with other non-terminal tree nodes, missing out on the opportunity to fuse and align sequence and structural information of source code well. Moreover, most complex tree-based or graph-based models suffer from low pre-processing and training efficiency \cite{Zonghan2021GNN} compared with sequence models.
% Existing methods either discard the code sequence or intersperse code tokens with other non-terminal tree nodes, losing the natural sequence format of the source code. 

% When using sequence models to process source code, we generally flatten the input source code to a token sequence where the nested hierarchical structure is implicitly expressed by indentations for languages such as Python or brackets for languages such as Java and C/C++. 
% It is sub-optimal to learn this information for sequence models.

% \TODO{模仿LEARNING TO REPRESENT PROGRAMS WITH GRAPHS中第一段里的写法}
In this work, we take a step to align structure information of programs with code sequences. Considering that the sequence model has been highly mature in NLP and other fields, our key insight is to retain the advantages of the sequence model such as computational efficiency, and add the structural information of the code at the minimum cost, therefore allow us to effectively solve source code processing tasks that are beyond the current state of the art.
% \TODO{need to refine}

% The hierarchical structure is essential in source code and influences the semantics of programs to a large extent.
% 现有的方法
% To tackle this issue in sequence modeling of source code,
% There have been some attempts to encode hierarchical information with sequence models, such as feeding the set of pairwise paths over AST \cite{code2vec, alon2018code2seq} or the traversal sequences of ASTs \cite{hu2018deep, SPTCode}.
% Others utilize tree-based models \cite{tbcnn,icseZhangWZ0WL19astnn,aaaiBuiYJ21treecaps} and graph-based models \cite{allamanis2018learning} to capture structural information.
% These methods 
% However, these methods either discard the code sequence or intersperse code tokens with other non-terminal tree nodes, losing the natural sequence format of the source code. 

% \TODO{need to refine}
% \TODO{这些方法增加了代码的结构信息，但其代价是损失了序列模型的优势，}
% \TODO{We focus on 怎样将这些hierarchical信息添加到序列模型中去，从而在发挥序列模型本身优势的前提下，同时学习到代码的结构特征，已实现更好效果的代码表示模型}
% \TODO{找到一种预处理方便，能在发挥序列模型本身优势的前提下，同时学习到代码的结构特征，已实现更好效果的代码表示模型}

% \TODO{Furthermore, modeling source code as a token sequence requires a minimum cost of pre-processing and is much more efficient than other data-flow-based or graph-based methods.}

To fully align structure and sequence information of programs, we analyze how the semantic structure influence the tokens in source code sequence and abstract it as a property of code tokens, called the hierarchical position.
% We claim that it is essential to simultaneously model the ``naturalness'' with sequence models and capture the ``hierarchy''.
% It cannot be ignored that most programming languages have hierarchical structures. 
% The semantics of programs are influenced by the hierarchical structure to a large extent.
We illustrate this influence from two aspects of the hierarchical position:
\ding{182} Hierarchical position of statements (named as \textit{\bf global hierarchy}).  The hierarchical position will affect the operational semantics of a statement. For example, in Figure \ref{fig:intro_locality}, the statement \definenode{count += 1} is written in the \definenode{for-block} and possibly to be executed more than once, while the statement \definenode{count = 0} will be executed only once in each function call to \definenode{countOccurrences}.
\ding{183} Hierarchical position of tokens within a statement (named as \textit{\bf local hierarchy}). Tokens are in different components in a statement, which will affect the semantics of each token. \Eg, as shown in Figure \ref{fig:locality}, \definenode{if-statement} contains \definenode{if-comparison} component and \definenode{if-block} component.
There are three identifiers, \textit{source\_i},  \textit{value}, and \textit{count}, in the \definenode{if-statement}. All of them are references to a variable in the function. However, the first two identifiers within \definenode{if-comparison} component (marked in green color in the figure) have more similar semantics than \textit{count} because they appear in the same comparison expression.
% When we flatten the input source code to a token sequence, 
% Therefore, we claim it is essential to model the hierarchy of programs in code sequence representation models.

% the distances between neighboring identifiers in the sequence are both 2 and we cannot directly identify the different roles of these three identifiers.
% 总结这个motivating
% 之前也有尝试加入结构信息的，SBT，但不好
% 如何综合考虑，同时考虑naturalness和hierarchy信息

% The hierarchical structure of source code is difficult for a simple sequence model to capture. When we flatten the input source code to a token sequence, the nested hierarchical structure is implicitly expressed by indentations for languages such as Python or brackets for languages such as Java and C/C++. We claim that it is important to model the hierarchy of programs in code understanding tasks and it is sub-optimal to learn this information from token sequences. 

To validate our intuition of modeling the sequential position and hierarchical position of code tokens, we propose to effectively unify hierarchical structure into the code sequence in a concise Transformer format, thus we name the network \textbf{Hi}erarchy \textbf{T}ransformer (HiT), a simple but effective model that can achieve a preferable balance between efficiency and effectiveness.
To extract the hierarchy of source code, we first parse the input code into a concrete syntax tree. The nested hierarchy can be represented by a path in the syntax tree. We use these syntax tree paths as additional hierarchical position to the sequence input. The HiT model consists of two key components: a Transformer-based hierarchy encoder that learns the representation of the hierarchical structure, and a Transformer-based sequence encoder that fuses the hierarchy information and token sequence information.

% Note that our model can be regarded as a general way to augment a sequence-based code understanding model. It is trivial and direct to extend our model to other sequence models such as RNN \cite{ZarembaSV14RNN} and LSTM \cite{HochreiterS97LSTM}. We choose Transformer \cite{vaswani2017attention} here because they have achieved state-of-the-art results in various NLP and source code-related tasks.

% Since Transformers have achieved state-of-the-art results in various NLP tasks, we make a small modification to the Transformer model and nest a small Transformer in the vanilla Transformer model. The locality representation for each token is added in a concise Transformer format.
We conduct an empirical study to investigate the impact of the global and local hierarchy. The experiment proves the effectiveness of the two different types of hierarchical position. It shows that with the cost of a small number of additional parameters, our approach significantly enhances the performance of sequence-based code representation models.
We further evaluate our approach on three tasks: code classification, clone detection, and method name prediction, with 8 different datasets from different domains. These tasks include classification tasks and generation tasks in the field of source code processing.
% , and both of them requires understanding the semantics of the input code snippets.
The experimental results show that our approach outperforms existing code representation models and other state-of-the-art models. With the additional hierarchical position, our approach enables sequential models to outperform even structure-based models such as graph-based or tree-based models. It indicates the benefits of our approach for combining the sequential and hierarchical position for source code understanding.

The main contributions of this paper are summarized as follows.
\begin{itemize}[leftmargin=*]
    \item We claim the influence of hierarchical position on the semantics of source code, which includes the hierarchy of the statements (named as global hierarchy) and the hierarchy within a statement (named as local hierarchy) in the code structure. The hierarchical position can be used as a bridge to align semantic structure and sequence information of source code.
    % The hierarchy information is complementary to the token sequence information of source code.
    \item We propose HiT, a simple but effective model to incorporate the hierarchical position into Transformer model. With the cost of a small number of additional parameters, our approach significantly improves the performance of code sequence representation models. We also conduct an empirical study exploring the effectiveness of the two different kinds of hierarchy information.
    \item We evaluate our approach on 3 source code-related tasks with 8 different datasets, involving classification tasks and generation tasks on source code. Our approach generally outperforms models on most of the tasks, showing excellent performance. Our experimental results prove that combining the sequential and hierarchical position is effective for learning representations for programs.
\end{itemize}

% Source code is formed by a sequence of one or more \textit{statements}, which performs as the syntactic unit. 
% The type of the \textit{\textbf{statement}} and its position in the program are different, and the components of the \textit{\textbf{token}} within the statement are also different. Due to the structure of programs, this 
% To this end, we propose the property of \textit{locality} of okens in code sequences.
% The locality of source code refers to the 
% The locality of source code refers to the fact that the semantic of a token or statement is related to the location and context. In other words, the locality determines the location and context information of a token in the code structure.
% Given a sequence of source code $s = [token_1, token_2, \dots, token_n]$, the same $token$ may have different locality, run in different environments/blocks, defined in different scopes, acted as different compositions and thus have very different semantic information. For the same reason, different tokens may also have more similar localities. For instance, Figure \ref{?} shows a piece of source code, illustrating the different changing relationships between token and locality.
% \TODO{add some explaination}
% def distance(x0, y0, x1, y1):
    % x0 = pow(abs(x0 - x1), 2)
    % y0 = pow(abs(y0 - y1), 2)
    % return sqrt(x0 + y0)



% \me{To tackle the issue of the "ambiguous" token in code sequence representation, } 
% To tackle the issue of tokens with unclear locality, we propose to explore the approach to incorporate locality into the sequence representation model of source code. We add additional locality information to each token so that the sequence representation of the code turns into $s^{new} = [(locality_1,token_1), (locality_2,token_2), \dots, (locality_n,token_n)]$.

% Thanks to the power of the sequence model,  it is an effective and direct approach to 
% Thanks to the powerfulness of deep learning, representations of code can be obtained via a variety of deep neural networks. 
% In order to obtain better code representations, researchers have incorporated structural information into the modeling process -- from the trivial token sequences \cite{DBLP:journals/neco/HochreiterS97,DBLP:conf/emnlp/ChoMGBBSB14}, to the abstract syntax trees (AST) \cite{DBLP:conf/aaai/MouLZWJ16,DBLP:conf/icse/ZhangWZ0WL19,DBLP:journals/pacmpl/AlonZLY19,alon2018code2seq} and finally to the graphs \cite{allamanis2018learning,fernandes2018structured,brockschmidt2018generative,yin2018learning,allamanis2020typilus}.


% 结合树结构信息的工作
% 在AST上的工作，以及在transformer上的处理
% Considering that the structural information of programming language is stronger than that of natural language, recently researchers are now focusing more on how to encode the structural information of programs in better ways. 
% Some studies use the flattened abstract syntax tree (AST) node sequence as input to model the structure in source code. SBT \cite{1} traverse an AST and represents the tree nodes into a token sequence, thus uses a sequential model such as LSTM to model the structure information. X-SBT \cite{1} simplifies the SBT approach, optimizing and shortening the length of the sequence representation by using an XML-like form. 
% \me{Some works leverage the program AST to model the structure in source code and linearize the graph by traversing it. Code2seq represents source code as a set of pairwise paths over AST where each path is compressed to a vector using LSTMs [Hochreiter and Schmidhuber, 1997]. Code2seq obtains state-of-the-art for code representation using only AST information, demonstrating the effectiveness of path encoding. }
% \me{On the other hand, several works also leverage structured graph neural networks for modelling source code directly. [Allamanis et al., 2017] used Gated Graph Neural Network (GGNN) to embed the semantically meaningful relationships in the code. [Zhou et al., 2019] proposed a novel graph neural network with composite programming representation for vulnerability identiﬁcation. However, GNNs typically rely on synchronous message passing, requiring message passing iterations to aggregate information [Allamanis et al., 2017, Fernandes et al., 2018]. Besides, primarily for computational reasons, GNNs for programs usually compute few message-passing iterations. For these reasons, the representation of GNNs tends to be local and struggle to leverage long-range interactions.}

% However, these studies meets some problems: Existing models lack the ability to combine lexical sequential information with structural hierarchical information. Both the flatten AST node sequence and the set of pairwise paths over AST impair or lose the sequence information of the context of the source code. In the flatten AST node sequence, the sequential information of leaf nodes (indicating the lexical sequential information) is interspersed with other non-terminal nodes. In Code2seq, the context of source code are ignored. As for GNNs, the number of nodes in the receptive field of each node grows exponentially, which leads to GNNs not being able to understand the complete sequence information and structure information well. 

% % 使用transformer编码树结构的既有工作，以及存在的问题
% There are also some studies devoted to representing structural information using Transformer models. 
% \me{Transformer [Vaswani et al., 2017] allows global information ﬂow at each step but lacks the ability to model the structural complexity of source code. Recently, some works have explored introducing structural inductive bias in Transformers to access the global structural representation of source codes. [Hellendoorn et al., 2019] proposed Graph Relation Embedding Attention Transformer (GREAT), which extends [Shaw et al., 2018] and biases Transformer with relational information from graph edge types. After that, [Zügner et al., 2021] proposed Code Transformer based on the backbone of XLNet in [Yang et al., 2019], which computes pairwise distances on AST and integrate multiple relations into the attention module.}

% To overcome these drawback shown in previous studies, we adopt the ideas of encoding path to represent source code and propose an effective approach, \method{}, which intergrate the \textbf{tree} structural information \textbf{in} sequential \textbf{Transformer} encoder-decoder architecture. In order to make the transformer model can handle both hierarchical and sequence information, we nest a new small Transformer in the vanilla Transformer model to process the hierarchical information.
% We employ root-to-leaf paths in AST to represent the hierarchical structural information.
% and use a small Transformer model to process these information.
% considering that leaf-to-leaf paths calculation is too complicated. (Given a full binary tree of depth $d$, the number of all leaf-to-leaf paths is $2^{2n-2}$) 
% These structural information is combined with the corresponding leaf nodes to form a sequence to process the lexical sequential information. 
% \TODO{}



==> chapter/related_deprecated.tex <==
\subsection{Deep Learning For Source Code Processing}

Deep learning techniques have been found useful in many software engineering tasks, such as code search \cite{husain2019codesearchnet}, code summarization \cite{DBLP:conf/acl/IyerKCZ16}, method name prediction \cite{allamanis2016convolutional,alon2018code2seq,DBLP:journals/pacmpl/AlonZLY19}, code completion \cite{DBLP:conf/msr/AllamanisS13a}, code classifiaction \cite{DBLP:conf/aaai/MouLZWJ16}, code clone detection \cite{DBLP:conf/icsm/SvajlenkoIKRM14,wang2020detecting}, \etc. 
These tasks can be largely divided into the two categories: classification tasks and generation tasks. 
\ding{182} Classification tasks require a transformed parameterized representation to distinguish in semantics. \citea{DBLP:conf/aaai/MouLZWJ16} proposed tree-based TBCNN for code classification. \citea{DBLP:conf/icse/ZhangWZ0WL19} proposed ASTNN for code representation based on AST, and applied it to code classification. \citea{hellendoorn2019global} proposed GREAT based on Transformer with relational information from code graphs and achieved good performances on classical classifcation tasks such as variable misuse.
\ding{183} Generations tasks generally require code snippets or nature language description as inputs and generate other sequential information associated with the program semantics. \citea{allamanis2016convolutional} proposed a convolutional attention networks to generate method names. \citea{hu2018deep} proposed DeepCom for code comment generation. \citea{DBLP:journals/pacmpl/AlonZLY19} and \citea{alon2018code2seq} proposed code2vec and code2seq for method name prediction. \citea{DBLP:conf/iclr/ZugnerKCLG21} proposed CodeTransformer to incorporate multiple relations to learning both structure and context jointly, boosting the results for several generation tasks. 
In this paper, we will conduct extensive experiments on classification and generation tasks, including method code classification, clone detection, method name prediction, so as to objectively evaluate the effectiveness of our approach.


\subsection{Structural Information in Code Representation Learning}
% v.s. code transformer % Our approach works in any programming language without complex preprocessing.

Code representation learning is a hot research topic in both software engineering and machine learning fields. 
% Different neural network-based approaches have been proposed for representing programs as vectors. 
Early research works learned language model on raw text data for code and used the source code token sequence as input \cite{DBLP:journals/corr/DamTP16,DBLP:conf/kbse/WangCMT16,allamanis2016convolutional,DBLP:conf/acl/IyerKCZ16}. However, programming languages have much stronger structural information than natural languages. Researchers are adopting different approaches to effectively encode these structural information, which can be divided into the following categories: 
(1) AST node sequence: \citea{hu2018deep} use the flattened AST node sequence as input. \citea{sptcode} use a XML-like form to simplify the SBT approach. 
(2) AST paths: \citea{alon2018code2seq} and \citea{code2vec} extracted paths from the AST for Java method naming, which encodes source code by regarding the set of paths as the representation of the AST.
(3) Trees-based or Graphs-based: \citea{DBLP:conf/aaai/MouLZWJ16} proposed tree-based convolutional neural networks to represent source code. \citea{allamanis2018learning} first proposed to use GGNN to represent programs graphs consisting of AST together with additional edges. 

Recently, there are also some studies integrating path representation of syntax tree into Transformer which show their capabilities in the field of code representation.
\citea{great} proposed Graph Relation Embedding Attention Transformer (GREAT), which extends [Shaw et al., 2018] and biases Transformer with relational information from graph edge types. \citea{DBLP:conf/iclr/ZugnerKCLG21} proposed Code Transformer based on the backbone of XLNet in [Yang et al., 2019], which computes pairwise distances on AST and integrate multiple relations into the attention module.

% \subsection{Sequence model?}

==> chapter/threats.tex <==
\paragraphwithoutdot{Threats to internal validity} relate to the roles of the model architecture and hyper-parameters setting.
In our experiments, we do a small-range grid search on learning rate and batch size settings. 
% We try to keep the hyper-parameters the same as baseline models for a fair comparison.
\zkc{add threats for GTNM not use context information}
\paragraphwithoutdot{Threats to external validity} mainly relate to tasks and datasets we choose. We counter this by evaluating our model on 8 different datasets of three tasks, including classification and generation tasks across 4 programming languages.

\paragraphwithoutdot{Threats to construct validity} include the evaluation metrics we used in this work. We utilize metrics of accuracy for code classification, MAP@R for clone detection, and precision, recall, F1 for method name prediction tasks. These metrics are adequate for corresponding tasks and have been adopted by many previous studies \cite{puri2021codenet,LuGRHSBCDJTLZSZ21codexglue,MusgraveBL20MAP,code2vec,alon2018code2seq,ZugnerKCLG21codetrans}.

==> table/results_clone.tex <==
\begin{table}[t]
% \footnotesize
    % \setlength\tabcolsep{3pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Results of models on code classification task \TODO{change to a bar figure like MISIM-GNN}}
\centering
\begin{tabular}{lc}
\hline
Model       & MAP@R \\ \toprule
code2vec    & 1.98  \\
code2seq    & 3.12  \\ \midrule
NCC         & 54.19 \\
Aroma       & 55.12 \\
TBCCD       & 23.42 \\ \midrule
MISIM-BoF   & 74.85 \\
MISIM-RNN   & 75.61 \\
MISIM-GNN   & 82.45 \\ \midrule
Transformer & 67.15 \\ \midrule
HiT         & 80.46 \\ \bottomrule
\end{tabular}

   \label{tab:res_clone}
\end{table}

==> table/results_with_hierarchy_abs_rel.tex <==
% \begin{table*}[t]
%   \centering
%   \caption{Results of Global vs. Local}
% \begin{tabular}{llccccccc}
% \toprule
%               &       & \multicolumn{5}{c}{\begin{tabular}[c]{@{}c@{}}Code Classification\\ (Accuracy)\end{tabular}}   & & \begin{tabular}[c]{@{}c@{}}Clone Detection \\ (MAP@R)\end{tabular} \\ \cline{3-7} \cline{9-9} 
%               & Para  & Java250 & Python800 & C++1000 & C++1400 & POJ-104 & & POJ-Clone                                   \\ \midrule
% \textbf{Ours} & 4.55M & 94.81   & 95.97     & 95.05   & 93.27   & 97.08   &                      & 80.46                                       \\
% Transformer   & 4.50M & 93.49   & 93.99     & 89.93   & 67.87   & 88.13   &                      & 67.15                                       \\ \midrule
% abs           & 4.55M & 93.79   & 94.84     & -       & -       & -       &                      & -                                           \\
% rel           & 4.55M & 93.95   & 95.42     & -       & -       & -       &                      & -                                           \\ \bottomrule
% \end{tabular}
  
%   \label{tab:with_hierarchy_abs_rel}
% \end{table*}

==> table/symbols.tex <==
\begin{table}[t] % \scriptsize
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Summary of notations and symbols in this paper.}
    \label{tab:notation}
    \begin{tabular}{ll}
    \toprule
Notation & Definition \\
    \midrule
% $\mathcal{D}^t,\mathcal{D}^v,\mathcal{D}^e$ & Train set, valid set \& eval set. \\
% $\mathcal{X},\mathcal{Y}$ & Source code space \& target space. \\
$\mathbf{s}=(t_1,\cdots,t_l)$ & Token sequence of the source code. \\
$\mathbf{e}=(e_1,\cdots,e_l)$ & Token embedding sequence. \\
$\mathbf{n}=(n_1,\cdots,n_{l'})$ & Node sequence in a tree path. \\
$\mathbf{p}=(p_1,\cdots,p_l)$ & Hierarchy representation for each code token. \\
% $M,\Theta_M$ & DL model \& its trainable parameters. \\
$W, b$ & Trainable parameters. \\
$y, \tilde y$ & Ground truth \& mode prediction. \\
$\mathcal{L}$ & Loss function. \\
% $Q,K,V$ & Query, key \& value in attention. \\
$h=(h_1,\cdots,h_{l})$ & Context-aware hidden representation. \\
    \bottomrule
    \end{tabular}
\end{table}
